Toxicity in Multilingual Machine Translation at Scale

Machine Translation systems can produce different types of errors, some of which are characterized as critical or catastrophic due to the specific negative impact that they can have on users. In this paper we focus on one type of critical error: added toxicity. We evaluate and analyze added toxicity when translating a large evaluation dataset (HOLISTICBIAS, over 472k sentences, covering 13 demographic axes) from English into 164 languages. An automatic toxicity evaluation shows that added toxicity across languages varies from 0% to 5%. The output languages with the most added toxicity tend to be low-resource ones, and the demographic axes with the most added toxicity include sexual orientation, gender and sex, and ability. We also perform human evaluation on a subset of 8 translation directions, confirming the prevalence of true added toxicity. We use a measurement of the amount of source contribution to the translation, where a low source contribution implies hallucination, to interpret what causes toxicity. Making use of the input attributions allows us to explain toxicity, because the source contributions significantly correlate with toxicity for 84% of languages studied. Given our findings, our recommendations to reduce added toxicity are to curate training data to avoid mistranslations, mitigate hallucination and check unstable translations.

==> figures/contributions.tex <==
\definecolor{color0}{HTML}{FFFFFF}
\definecolor{color1}{HTML}{FFEDE5}
\definecolor{color2}{HTML}{FEE5D8}
\definecolor{color3}{HTML}{FED9C9}
\definecolor{color4}{HTML}{FDCAB5}
\definecolor{color5}{HTML}{FCBBA1}




\newcommand*{\mybox}[2]{{\setlength{\fboxsep}{0.15pt}\colorbox{#1}{\strut #2}}}


%\newcommand*{\mybox}[2]{\tikz[anchor=base,baseline=0pt,rounded corners=0pt, inner sep=0.2mm] %\node[fill=#1!60!white] (X) {#2};}
%\newcommand*{\mybbox}[2]{\tikz[anchor=base,baseline=0pt,inner sep=0.2mm,] %\node[draw=black,thick,fill=#1!60!white] (X) {#2};}

\begin{figure}
\centering
\begin{tabular}{@{}p{13.5cm}@{\hspace{0.2cm}}p{13.5cm}@{}}
%  \resizebox{0.49\textwidth}{!}{%
  \small 
 \textbf{Hallucination}\\
 \midrule
 \small Sentence 1 \\ 
 \small
 \mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{I}} \mybox{color0}{\strut{love}} \mybox{color0}{\strut{being}} \mybox{color4}{\strut{chubby.}} \mybox{color0}{\strut{$<$/s$>$}}  \mybox{color0}{\strut{$<$/s$>$}} \mybox{color1}{\strut{$\_$$\_$fra$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{J'adore}} \mybox{color0}{\strut{être}} \mybox{color2}{\strut{une}} \mybox{color5}{\strut{grosse}} \mybox{color0}{\strut{\bf{chatte}.}}\\ %part8 unfiltered 9564
  \midrule
  \small 
 \textbf{Mistranslation}\\
 \midrule
 \small Sentence 2 \\
 \midrule
 \small
 \mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hi!}} \mybox{color0}{\strut{I'm}} \mybox{color0}{\strut{a}} \mybox{color5}{\strut{gangly}} \mybox{color1}{\strut{child.}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color4}{\strut{$\_$$\_$cat$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hola,}} \mybox{color0}{\strut{sóc}} \mybox{color0}{\strut{un}} \mybox{color4}{\strut{nen}} \mybox{color0}{\strut{\bf{malparit}.}}\\
  \midrule
  \small
%\textbf{Semantically related translation, wrong level of offensiveness}\\
%\midrule
% \small Sentence 3 \\
% \midrule
% \small
% \mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hi}} \mybox{color0}{\strut{I'm}} \mybox{color0}{\strut{a}} \mybox{color5}{\strut{queer}} \mybox{color2}{\strut{sibling.}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color1}{\strut{$\_$$\_$spa$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hola}} \mybox{color0}{\strut{soy}} \mybox{color0}{\strut{un}} \mybox{color2}{\strut{hermano}} \mybox{color0}{\strut{\bf{marica}.}}\\
%\mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} %\mybox{color0}{\strut{I'm}} \mybox{color0}{\strut{not}} %\mybox{color0}{\strut{a}} \mybox{color5}{\strut{queer}} %\mybox{color1}{\strut{guy.}} \mybox{color0}{\strut{$<$/s$>$}} %\mybox{color0}{\strut{$<$/s$>$}} %\mybox{color3}{\strut{$\_$$\_$cat$\_$Latn$\_$$\_$}} %\mybox{color0}{\strut{No}} \mybox{color0}{\strut{sóc}} %\mybox{color0}{\strut{un}} \mybox{color2}{\strut{tipus}} %\mybox{color0}{\strut{\bf{maricona}.}}\\
% \midrule
% \small
 %\textbf{Semantically related translation, correct level of offensiveness}\\
 \textbf{Correct translation}\\
\midrule
 \small Sentence 3 \\
 \midrule
 \small
%  \mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hi!}} \mybox{color0}{\strut{I'm}} \mybox{color0}{\strut{a}} \mybox{color0}{\strut{person}} \mybox{color0}{\strut{with}} \mybox{color5}{\strut{dyslexia.}} \mybox{color0}{\strut{</s>}} \mybox{color0}{\strut{</s>}} \mybox{color2}{\strut{$\_$$\_$cat$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hola!}} \mybox{color0}{\strut{Sóc}} \mybox{color0}{\strut{una}} \mybox{color0}{\strut{persona}} \mybox{color3}{\strut{amb}} \mybox{color0}{\strut{dislèxia.}}\\
   \mybox{color0}{\strut{$\_$$\_$eng$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hi!}} \mybox{color1}{\strut{I'm}} \mybox{color0}{\strut{a}} \mybox{color5}{\strut{50-year-old}} \mybox{color1}{\strut{woman.}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color0}{\strut{$<$/s$>$}} \mybox{color3}{\strut{$\_$$\_$cat$\_$Latn$\_$$\_$}} \mybox{color0}{\strut{Hola,}} \mybox{color0}{\strut{sóc}} \mybox{color0}{\strut{una}} \mybox{color3}{\strut{dona}} \mybox{color0}{\strut{de}} \mybox{color0}{\strut{\bf{50}}} \mybox{color0}{\strut{\bf{anys}.}}\\
\midrule

  \end{tabular}
  \caption{Examples of translations in English-to-French, English-to-Spanish or English-to-Catalan.
  %Each sentence shows the input attribution to the word in bold  
  Sentences show input attributions for bold words in the cases of hallucination (sentence 1); mistranslation (sentence 2); %a semantically related translation but wrong level of offensiveness (sentence 3); 
  and a correct translation (sentence 3).  We observe that the hallucination example focuses more in the target context than in the source sentence compared to the other two examples. \label{fig:hallucinationmistranslation}}
\end{figure}

